Generalization in Supervised Learning Through Riemannian Contraction

We prove that Riemannian contraction in a supervised learning setting implies generalization. Specifically, we show that if an optimizer is contracting in some Riemannian metric with rate $\lambda > 0$, it is uniformly algorithmically stable with rate $\mathcal{O}(1/\lambda n)$, where $n$ is the number of labelled examples in the training set. The results hold for stochastic and deterministic optimization, in both continuous and discrete-time, for convex and non-convex loss surfaces. The associated generalization bounds reduce to well-known results in the particular case of gradient descent over convex or strongly convex loss surfaces. They can be shown to be optimal in certain linear settings, such as kernel ridge regression under gradient flow.

==> scraps.tex <==
Here the algorithm is:

\[\mathcal{A}(S) = \text{arg}\min_{\theta}{R_S[\theta]} \]

We will also define the following quantity which will be helpful, the incremental output of algorithm $\mathcal{A}_t(S)$, which is the value of $\theta$ returned by the optimization algorithm time $t$ (or step $t$, in discrete time). In the case of an optimization algorithm which is proven to have a global, globally stable minimizer, we have:

\[\lim_{t \rightarrow \infty} \mathcal{A}_t(S) =  \mathcal{A}(S) \]


Similarly, we define the \textit{incremental} generalization gap, which is the generalization gap with respect to the output of the optimization algorithm stopped at time $t$:

\[\Delta^{gen}_{inc} (\theta(t)) \equiv R[\theta(t)] - R_S[\theta(t)] \]

Which yields:

\[\lim_{t \rightarrow \infty} \Delta^{gen}_{inc} (\theta(t)) =  \Delta^{gen} \]


Consider the following training rule applied to the parameter vector $\theta \in \mathbb{R}^p$ on training set $S$:


\[\dot{\theta} = h(\theta,S) \]

And the same rule applied on training set $S^{(i)}$ can be decomposed as:

\[\dot{\theta'} = h(\theta',S) + u(z_i,z'_i,\theta') \]

And the dynamics $h$ is contracting in the identity metric, then we have by the robustness result that, after exponential transients:

\[||\theta' - \theta|| \leq \frac{||u(z_i,z'_i,\theta')||}{\lambda}\]

Thus if $||u(z_i,z'_i,\theta')||$ is a decreasing function of $n$, we will have $\theta' \rightarrow \theta$ as $n \rightarrow \infty$.


\[|\ell((A(S^{(i})),z_i) - \ell((A(S),z_i)| =  |\ell(\theta',z_i) - \ell(\theta,z_i)| \leq L||\theta' - \theta||\]

Consider as an example the case of empirical risk minimization through gradient descent on the empirical loss function. In this case we have:

\[\dot{\theta} = - \frac{1}{n}\sum^{n}_{i =1}\nabla \ell(f(\theta,x_i),y_i)  \]

\[\dot{\theta'} = -\frac{1}{n}\sum^{n}_{i = 1}\nabla \ell(f(\theta',x_i),y_i) -  \frac{1}{n}(\ell(f(\theta',x_i),y_i) + \ell(f(\theta',x'_i),y'_i)) \]

Thus, we have:

\[u(z_i,z'_i,\theta') = \frac{1}{n}(\ell(f(\theta',x_i),y_i) + \ell(f(\theta',x'_i),y'_i)) \]

Which implies that 

\[||\theta' - \theta|| \leq \mathcal{O}(\frac{1}{n\lambda})\]

This in turn implies that:


\[||\ell(\theta',z_i) - \ell(\theta,z_i)|| \leq \mathcal{O}(\frac{1}{n\lambda}) \]

Which in turn implies that $\mathcal{A}$ generalizes well, since:

\[ \Delta_{gen}(f) \leq \mathcal{O}(\frac{1}{n\lambda}) \]





%proof of partial contraction robustness
\begin{proof}
Consider the auxiliary, perturbed system:

\[ \dot{\mathbf{y}_p} = \mathbf{g}(\mathbf{y}_p,\mathbf{x}_p,t) + \mathbf{d}(\mathbf{x}_p,t)\]

Since the unperturbed auxillary system is assumed to be contracting, we know from Theorem \ref{theorem:contraction_robustness} that \textit{any} trajectory of $\mathbf{y}_p$ satisfies:

\[||\mathbf{y} - \mathbf{y}_p|| \leq \chi e^{-\lambda t}||\mathbf{y}(0) - \mathbf{y}_p(0)|| + \frac{d \chi}{\lambda}  \]

since $\mathbf{x}_p(t)$ is a particular trajectory of the disturbed auxillary system, we have:

\[||\mathbf{y} - \mathbf{x}_p|| \leq \chi e^{-\lambda t}||\mathbf{y}(0) - \mathbf{x}_p(0)|| + \frac{d \chi}{\lambda}  \]

Of course we also know that the unperturbed system verifies:

\[||\mathbf{x} - \mathbf{y}|| \leq \chi e^{-\lambda t}||\mathbf{x}(0) - \mathbf{y}(0)|| \]

Finally, we have via the triangle inequality that:

\[||\mathbf{x} - \mathbf{x}_p|| \leq \chi e^{-\lambda t} (||\mathbf{x}(0) - \mathbf{y}(0)|| + ||\mathbf{y}(0) - \mathbf{y}_p(0)||) + \frac{d \chi}{\lambda}  \]

which proves the result.

\end{proof}



\subsection{Stochastic Gradient Descent}
\subsubsection{Discrete-Time SGD}
So far we have been describing batch gradient descent. However far more often one uses mini-batch gradient descent, which requires a different analysis. We approach this in two ways. First of all, the main results of contraction analysis (in particular robustness) all have discrete-time analogous. So we can directly apply it to the case of stochastic gradient descent:

Consider the stochastic update:

\[ \theta_{t+1} = \theta_{t} +  \alpha_t\mathbf{g}(\theta,z_i)\]

And assume that the system is discrete-time contracting in expectation, in the sense that:

\[	\mathbb{E} \mathbf{J}^T\mathbf{M}\mathbf{J} - \mathbf{M} \leq -2\lambda \mathbf{M} 	\rangle\]


An analogous result also holds for the discrete-time dynamics:



In this case the contraction conditions becomes:


Similarly, for \eqref{eq:dynamical_system_discrete}, if the following discrete-time differential Lyapunov equation is satisfied:

\begin{equation}\label{eq:disc_contraction_equation}
\mathbf{J}_t^T\mathbf{M}_{t+1}\mathbf{J}_t - \mathbf{M}_t \leq -2\lambda\mathbf{M}_t
\end{equation}

or the discrete-time dynamics:
\begin{equation}\label{eq:dynamical_system_discrete}
\mathbf{x}_{t+1} = \mathbf{f}(\mathbf{x}_t,t)
\end{equation}


\section{Double Descent As Dynamical Overshoot}
In this section we speculate that the empirically observed double-descent could be a consequence of an optimizer which is contracting in a poorly conditioned metric. Consider a generic algorithmic stability bound of the form we have been dealing with throughout the paper:

\[ \epsilon_{stab} \leq \chi L e^{-\lambda t}||\mathbf{\theta}_S(0)-\mathbf{\theta}_{S'}(0)|| + \frac{2\chi L \xi}{\lambda n} \]
focusing on the exponential-decaying term, notice that the presence of the metric and Lipshitz constant imply the possibility of \textit{overshoot}. In particular, at fixed $n$ and $t = 0$ we have that our algorithmic-stability bound is strictly worse than $\epsilon_{stab} = L ||\theta(0) - \theta_p(0)||$. As training goes on, the exponential term eventually forces our bound to be better. 


\affil[2]{Department of Mechanical Engineering, MIT}


Loss landscapes characterized by PL* may have infinitely many global minima . Because of this we cannot expect gradient descent on these landscapes to be contracting, since two optimizer trajectories initialized at different minima would stay there indefinitely (and thus not converge towards each other). Furthermore, these loss landscapes are generically not even locally convex around equilibrium points \citep{liu2021loss}, so we cannot apply the results from Section \ref{subsubsection:convexlossesGD}.



 In this case $V_{S'}$ can be written as a perturbed version of $V$ by again using the decomposition:

\[\nabla \mathcal{L}_{S'}(\boldsymbol{\theta}_{S'}) = \nabla \mathcal{L}_{S}(\boldsymbol{\theta}_{S'}) - \mathbf{p} \]
where $\mathbf{p} \equiv \frac{1}{n}(\nabla \ell(\boldsymbol{\theta}_{S'},z_i) - \nabla \ell(\boldsymbol{\theta}_{S'},z'_i))$. From this it follows that:

\begin{align}
\dot{V}_{S'} = \nabla \mathcal{L}_{S'}(\boldsymbol{\theta}_{S'})^T\boldsymbol{\dot{\theta}}_{S'} = -(\nabla \mathcal{L}_{S}(\boldsymbol{\theta}_{S'}) - \mathbf{p})^T(\nabla\mathcal{L}_{S}(\boldsymbol{\theta}_{S'}) - \mathbf{p})   \\
 = -||\nabla \mathcal{L}_{S}(\boldsymbol{\theta}_{S'})||^2 + d
\end{align}
which may be viewed as a perturbed version of the $V_S$ dynamics with disturbance term: $d \equiv 2\mathbf{p}^T\nabla \mathcal{L}_{S}(\boldsymbol{\theta}_{S'}) - \mathbf{p}^T\mathbf{p}$. 



Note that the norm of $d$ is upper-bounded as follows:
\[ |d| \leq 2||\mathbf{p}||L - ||\mathbf{p}||^2 \leq \frac{4L^2}{n} \]
Since $V_{S} = \mathcal{L}_S(\theta_{S}) \rightarrow 0$ exponentially with rate $\mu$ and $V_{S'}$ converges to a ball of radius $|d|/\mu$ around the origin, this implies that:
\[\epsilon_{stab} =  \frac{4L^2}{\mu n} \]
where we have used the fact that as $t \rightarrow \infty$:
\[\mathbb{E}_S|\ell(\boldsymbol{\theta}_{S'},z_i) - \ell(\boldsymbol{\theta}_{S},z_i) | = \mathbb{E}_S|\ell(\boldsymbol{\theta}_{S'},z_i)| \leq \mathbb{E}_S|\mathcal{L}_{S'}(\boldsymbol{\theta}_{S'})|  \leq \frac{4L^2}{\mu}(\frac{1}{n} + \frac{1}{n^2}) \]
where the last inequality is verified after exponential transients of rate $\mu$.

\begin{remark}[PL* on Manifolds]
The analysis in the preceding section can be readily applied to natural gradient descent on a loss landscape which satisfies the PL* condition defined on a Riemannian manifold with metric $\mathbf{M}(\boldsymbol{\theta},t)$. In particular consider a loss surface which satisfies:

\[\nabla \mathcal{L}^T(\boldsymbol{\theta})\mathbf{M}(\boldsymbol{\theta},t)\nabla \mathcal{L}(\boldsymbol{\theta}) \geq \mu\mathcal{L}(\boldsymbol{\theta})\]
and the natural gradient descent:
\[\boldsymbol{\dot{\theta}} = - \mathbf{M}(\boldsymbol{\theta},t)\nabla \mathcal{L} \]
Using the Lyapunov function $V = \mathcal{L}$ yields the same analysis as in the preceding subsection, with $V$ converging to zero exponentially with rate $\mu$. A loss surface that satisfies the above Riemannian PL* condition also satisfies the original PL* condition, meaning that if one uses `regular' gradient descent:
\[\boldsymbol{\dot{\theta}} = - \nabla \mathcal{L} \]
then the result still holds, but $\mu \rightarrow \frac{\mu}{\sigma_{max}(\mathbf{M})}$, where $\sigma_{max}$ denotes the largest singular value. This is because:

\[\sigma_{max}(\mathbf{M}) ||\nabla \mathcal{L}||^2 \geq \nabla \mathcal{L}^T(\boldsymbol{\theta})\mathbf{M}(\boldsymbol{\theta},t)\nabla \mathcal{L}(\boldsymbol{\theta}) \geq \mu\mathcal{L}(\boldsymbol{\theta})\]
implying that:
\[||\nabla \mathcal{L}||^2 \geq \frac{\mu}{\sigma_{max}(\mathbf{M})}\mathcal{L}(\boldsymbol{\theta})\]
which is just the original PL* condition with scaled $\mu$.
\end{remark}

We also assume that $V$ is radially unbounded, in the sense that $V \rightarrow \infty$ as $||\boldsymbol{\theta}|| \rightarrow \infty$.


\subsubsection{Lyapunov Functions}
\label{subsubsection: PL}
Constructing a Lyapunov function to prove optimizer stability is sometimes easier than finding a contraction metric \citep{jouffroy2010tutorial}. Here we show that under certain conditions Lyapunov stability of the optimizer is sufficient for controlling its generalization error. In particular, consider a Lyapunov function $V$ which goes to zero as $t \rightarrow \infty$ and satisfies a quadratic growth bound:

\[V(\boldsymbol{\theta}) \geq \mu ||\boldsymbol{\theta} - \boldsymbol{\theta}^*||^2\]
where $V(\boldsymbol{\theta}) = 0 \iff \boldsymbol{\theta} = \boldsymbol{\theta}^*$ and $\mu>0$. In the case where multiple global minimizers of $V$ might exist, $\boldsymbol{\theta}^*$ denotes the Euclidean projection of $\boldsymbol{\theta}$ onto the set of global minimizers. Note that via \eqref{eq:lip_ass}, to control the generalization error it is sufficient to control $||\boldsymbol{\theta}_{S'} - \boldsymbol{\theta}^*_{S}||$, because :
\[||\boldsymbol{\theta}_{S} -\boldsymbol{\theta}_{S'}|| \leq ||\boldsymbol{\theta}_{S} - \boldsymbol{\theta}^*_{S} || + ||\boldsymbol{\theta}_{S'} - \boldsymbol{\theta}^*_{S}||  \] 
Since $||\boldsymbol{\theta}_{S} - \boldsymbol{\theta}^*_{S} ||$ goes to zero by assumption, we need to obtain bounds for $||\boldsymbol{\theta}_{S'} - \boldsymbol{\theta}^*_{S}||$. To do this we use classical results from nonlinear control theory \citep{Khalil:1173048} which bound the behavior of a perturbed system by using the stability of a nominal, unperturbed system. As in Theorem \eqref{theorem:Contraction_Implies_AS} we consider the optimizer dynamics over set $S$ to be unperturbed and the same optimizer dynamics over set $S'$ to be perturbed. In particular:

\[\boldsymbol{\dot{\theta}_S} = \mathbf{G}(\boldsymbol{\theta}_S,S) \]

\[\boldsymbol{\dot{\theta}}_{S'} = \mathbf{G}(\boldsymbol{\theta}_{S'},S') = \mathbf{G}(\boldsymbol{\theta}_{S'},S) + \mathbf{p} \]
where $||\mathbf{p}||\leq p = \frac{2\xi}{n}$ is the disturbance term. In addition to the quadratic growth bound, we assume the following:
\[\dot{V} = \frac{\partial V}{\partial t} + \frac{\partial V}{\partial \boldsymbol{\theta}}\mathbf{G}(\boldsymbol{\theta},S) \leq - \beta V  \hspace{0.5cm} \forall t,\boldsymbol{\theta}\]

\[ ||\frac{\partial V}{\partial \boldsymbol{\theta} }|| \leq M \]
The first inequality implies exponential stability of the optimizer dynamics, and the second assumption implies that the Lyapunov function is $M$-Lipshitz. Now consider the evolution of $V$ along trajectories of $\boldsymbol{\theta}_{S'}$:

\[\dot{V}(\boldsymbol{\theta}_{S'}) = \frac{\partial V}{\partial t} + \frac{\partial V}{\partial \boldsymbol{\theta}_{S'}}\mathbf{G}(\boldsymbol{\theta}_{S'},S) + \frac{\partial V}{\partial \boldsymbol{\theta}_{S'}}\mathbf{p}  \leq - \beta V(\boldsymbol{\theta}_{S'}) + Mp \]
This implies that $V(\boldsymbol{\theta}_{S'})$ is upper-bounded as follows:
\[V(\boldsymbol{\theta}_{S'}) \leq V(\boldsymbol{\theta}_{S'}(0))e^{-\beta t} + \frac{M p}{\beta}\]
Combining this with the quadratic growth inequality and substituting in $p =\frac{2\xi}{n}$ yields:
\[||\boldsymbol{\theta}_{S'} - \boldsymbol{\theta}^*_S||^{2} \leq V(\boldsymbol{\theta}_{S'}(0))e^{-\beta t} + \frac{2M \xi}{n\beta \mu } \]
which implies a generalization error that scales at least as quickly as $\frac{1}{\sqrt{n}}$. If instead of the quadratic lower bound $V$ satisfied, for example, a norm lower bound:

\[V(\boldsymbol{\theta}) \geq \mu ||\boldsymbol{\theta} - \boldsymbol{\theta}^*_S||\]
the generalization error would scale with $\frac{1}{n}$.

\begin{remark}[Polyak-Lojasiewicz (PL) Condition]
Several recent papers have argued that overparameterized deep neural networks have loss surfaces which satisfy the Polyak-Lojasiewicz (PL) Condition \citep{polyak1963gradient,oymak2019overparameterized,bassily2018exponential,liu2021loss}:
\[||\nabla \mathcal{L}(\boldsymbol{\theta})||^2 \geq \mu(\mathcal{L}(\boldsymbol{\theta}) - \mathcal{L}(\boldsymbol{\theta}^*)) \hspace{.5cm} \forall \hspace{.1cm} \boldsymbol{\theta} \in \mathcal{C}\]
where $\mu > 0$ and $\mathcal{C}$ is a set.  Consider the gradient flow:
\[\boldsymbol{\dot{\theta}} = - \nabla \mathcal{L}(\boldsymbol{\theta}) \]
As pointed out in \cite{wensing2020beyond}, the PL-condition allows us to use the empirical residual loss as a Lyapunov function (i.e $V = \mathcal{L} - \mathcal{L}^*$), because:
\[\dot{V} = \nabla \mathcal{L}^T\boldsymbol{\dot{\theta}} = -||\nabla \mathcal{L}(\boldsymbol{\theta})||^2 \leq -\mu V  \]
Additionally, as was proven in \cite{karimi2016linear} and later used by \cite{charles2018stability} the PL condition implies the quadratic growth condition:

\[\mathcal{L}- \mathcal{L}^* \geq \frac{\mu}{2}||\boldsymbol{\theta}-\boldsymbol{\theta}^* ||^2 \]
together with the observation that $||\frac{\partial V}{\partial \boldsymbol{\theta}}|| \leq L$ (and thus $M = L$), the results of the preceding section allow us to conclude that gradient flows over a loss surface which is PL have vanishing generalization error with increasing $n$.

\end{remark}


Consider the differential displacement $\delta \mathbf{x}$ and the local coordinate transforms $\mathbf{T}_1(\mathbf{x},t)$ and $\mathbf{T}_2(\mathbf{x},t)$:

\[\delta \mathbf{z}_1 = \mathbf{T}_1\delta \mathbf{x} \]
\[\delta \mathbf{z}_2 = \mathbf{T}_2 \delta \mathbf{x} = \mathbf{T}_2 \mathbf{T}^{-1}_1 \delta \mathbf{z}_1 \]
The geodesic distance between two points $P_1$ and $P_2$ with respect to metric $\mathbf{M}$ is the smallest path integral $R = \int_{P_1}^{P_2} ||\delta \mathbf{z}||_2$. The geodesic distance computed with respect to $\mathcal{M}_2$ may be upper-bounded and lower bounded as follows:

\[k_1 \int_{P_1}^{P_2}  ||\delta \mathbf{z}_1||_2  \leq \int_{P_1}^{P_2} ||\delta \mathbf{z}_2||_2 \leq  k_2 \int_{P_1}^{P_2}  ||\delta \mathbf{z}_1||_2\]
or, equivalently:

\[0 < k_1  \leq \frac{d_{\mathcal{M}_2}(P_1,P_2)}{d_{\mathcal{M}_1}(P_1,P_2)} \leq  k_2 \]
where $k_1$, $k_2$ denote uniform lower and upper bounds on the singular values of $\mathbf{T}_2 \mathbf{T}^{-1}_1$.







\begin{lemma}
More generally, if we could guarantee contraction in metric $\mathbf{M}_1$ but were measuring robustness in $\mathbf{M}_2$, then $\chi \rightarrow \sigma_{max}({\mathbf{T}_2})\chi$, where $\sigma_{max}(\cdot)$ denotes the largest singular value.
\end{lemma}

\begin{proof}
If $R_I$ is bounded, then:

\[ R_I \leq C \]
This immediately implies that $R_2 \equiv ||\mathbf{T}_2(\mathbf{x} - \mathbf{x}_p)|| \leq C\sigma_{max}({\mathbf{T}_2})$, because:
\[\frac{R_2}{\sigma_{max}({\mathbf{T}_2})} \leq R_I \leq C\]
Thus, if \eqref{eq:contraction_robustness_equation} is satisfied, then:

\[R_2 \leq \sigma_{max}({\mathbf{T}_2})\chi R_I(0)e^{-\lambda t} + \frac{d \sigma_{max}({\mathbf{T}_2}) \chi}{\lambda} \]
which proves the result.

\end{proof}

%Generalization in Supervised Learning Through Riemannian Contraction
%Riemannian Contraction Provides Generalization Bounds in Supervised Learning
% Riemannian Contracting Optimizers Certify Algorithmically Stable Supervised Learning? 
